HD 83443c: A highly eccentric giant planet on a 22-year orbit

We report the discovery of a highly eccentric long-period Jovian planet orbiting the hot-Jupiter host HD\,83443. By combining radial velocity data from four instruments (AAT/UCLES, Keck/HIRES, HARPS, Minerva-Australis) spanning more than two decades, we find evidence for a planet with m~sin~$i=1.35^{+0.07}_{-0.06}$\,\mj, moving on an orbit with $a=8.0\pm$0.8\,au and eccentricity $e=0.76\pm$0.05. We combine our radial velocity analysis with \textit{Gaia} eDR3 /\textit{Hipparcos} proper motion anomalies and derive a dynamical mass of $1.5^{+0.5}_{-0.2} M_{\rm Jup}$. We perform a detailed dynamical simulation that reveals locations of stability within the system that may harbor additional planets, including stable regions within the habitable zone of the host star. HD\,83443 is a rare example of a system hosting a hot Jupiter and an exterior planetary companion. The high eccentricity of HD\,83443c suggests that a scattering event may have sent the hot Jupiter to its close orbit while leaving the outer planet on a wide and eccentric path.

==> Online_long_table.tex <==
% Make this a long table with all RVs in one table.  Do we want a stub table?
\startlongtable
\begin{deluxetable}{cccc}
\tabletypesize{\scriptsize}
\tablecaption{Radial Velocities for HD\,83443}
\label{tab:allRV}
\tablehead{
\colhead{Time} & \colhead{Velocity} & \colhead{Uncertainty} & \colhead{Instrument}\\
\colhead{[BJD]} & \colhead{[\mos]} & \colhead{[\mos]} & \colhead{}}
\startdata
%         :        &     :    &   :    & : \vspace{4pt} \\
  \multicolumn4c{{\textsc{Minerva}}-Australis - ThAr} \\
2458523.05882338 & 28316.1248 & 8.88 & {\textsc{Minerva}}-ThAr  \\
2458523.06634676 & 28292.2683 & 7.54 & {\textsc{Minerva}}-ThAr  \\
2458527.22736930 & 28176.2535 & 10.04 & {\textsc{Minerva}}-ThAr  \\
2458527.23836497 & 28196.2810 & 7.24 & {\textsc{Minerva}}-ThAr  \\
2458530.13194543 & 28196.9606 & 7.77 & {\textsc{Minerva}}-ThAr  \\
2458530.14292949 & 28216.8482 & 9.29 & {\textsc{Minerva}}-ThAr  \\
2458532.19110159 & 28248.3593 & 7.11 & {\textsc{Minerva}}-ThAr  \\
2458532.20209720 & 28263.8133 & 10.75 & {\textsc{Minerva}}-ThAr  \\
2458533.20590349 & 28219.9088 & 13.91 & {\textsc{Minerva}}-ThAr  \\
2458534.13895505 & 28283.3215 & 7.60 & {\textsc{Minerva}}-ThAr  \\
2458534.14995064 & 28274.9733 & 8.34 & {\textsc{Minerva}}-ThAr  \\
2458537.11840857 & 28280.5237 & 8.43 & {\textsc{Minerva}}-ThAr  \\
2458537.13287641 & 28285.8933 & 9.02 & {\textsc{Minerva}}-ThAr  \\
2458537.14733267 & 28288.8329 & 13.65 & {\textsc{Minerva}}-ThAr  \\
2458538.15112244 & 28273.0829 & 9.59 & {\textsc{Minerva}}-ThAr  \\
2458538.16211799 & 28263.8454 & 8.40 & {\textsc{Minerva}}-ThAr  \\
2458538.17310196 & 28262.0201 & 9.71 & {\textsc{Minerva}}-ThAr  \\
\hline
 \multicolumn4c{{\textsc{Minerva}}-Australis - Iodine} \\
 2459262.95634463 & 28268.8694 & 7.04 & {\textsc{Minerva}}-Iodine  \\
2459263.13735550 & 28247.5282 & 8.86 & {\textsc{Minerva}}-Iodine  \\
2459267.01451502 & 28191.8134 & 8.00 & {\textsc{Minerva}}-Iodine  \\
2459267.95635994 & 28184.3384 & 13.61 & {\textsc{Minerva}}-Iodine  \\
2459267.99196239 & 28175.6199 & 12.10 & {\textsc{Minerva}}-Iodine  \\
  \hline
  \multicolumn4c{HARPS-pre correction} \\
2453001.85140 & 54.062 & 0.917 & HARPS \\
2453015.78017 & -47.280 & 0.938 & HARPS \\
2453031.67569 & 50.459 & 0.665 & HARPS \\
2453031.76855 & 56.922 & 0.638 & HARPS \\
2453031.87649 & 64.873 & 0.714 & HARPS \\
2453033.64667 & -44.503 & 0.936 & HARPS \\
2453033.74475 & -40.663 & 0.917 & HARPS \\
2453033.87367 & -35.924 & 0.932 & HARPS \\
2453047.71388 & 7.530 & 0.980 & HARPS \\
2453048.71702 & -44.067 & 0.948 & HARPS \\
2453050.72817 & 3.706 & 0.956 & HARPS \\
2453052.65757 & 49.349 & 0.877 & HARPS \\
2453056.67167 & 7.434 & 0.944 & HARPS \\
2453058.75400 & 60.552 & 1.044 & HARPS \\
2453059.72894 & 0.867 & 0.970 & HARPS \\
2453060.67451 & -40.513 & 0.965 & HARPS \\
2453064.70721 & 63.342 & 0.941 & HARPS \\
2453866.54501 & -41.868 & 0.922 & HARPS \\
2454843.82819 & 7.261 & 0.964 & HARPS \\
2454844.80115 & 9.616 & 0.998 & HARPS \\
2454845.73377 & -75.951 & 1.088 & HARPS \\
2454845.86659 & -77.818 & 0.980 & HARPS \\
2454846.73997 & -3.088 & 0.941 & HARPS \\
2455288.60700 & -2.626 & 0.675 & HARPS \\
2455298.58846 & 11.490 & 0.835 & HARPS \\
2455527.86126 & 36.297 & 0.880 & HARPS \\
2456723.62454 & -58.910 & 0.647 & HARPS \\
2456725.59758 & 39.138 & 0.608 & HARPS \\
2456727.63578 & 7.350 & 0.555 & HARPS \\
2456740.57622 & 36.258 & 0.790 & HARPS \\
2456744.73750 & -61.675 & 0.736 & HARPS \\
2456748.62640 & 18.622 & 0.694 & HARPS \\
2456758.61417 & 23.949 & 0.871 & HARPS \\
2457033.74759 & -30.269 & 0.953 & HARPS \\
2457036.80175 & -38.490 & 0.642 & HARPS \\
2457044.73787 & 50.404 & 1.000 & HARPS \\
2457048.70384 & -33.209 & 0.739 & HARPS \\
2457062.77181 & 50.433 & 0.741 & HARPS \\
2457064.81246 & -15.902 & 0.656 & HARPS \\
2457114.67921 & -55.002 & 0.736 & HARPS \\
2457116.66409 & 41.078 & 0.728 & HARPS \\
2457117.65796 & -55.118 & 0.690 & HARPS \\
2457138.58973 & -56.921 & 0.766 & HARPS \\
2457139.59119 & 2.752 & 0.958 & HARPS \\
2457143.63103 & 36.516 & 0.754 & HARPS \\
 \hline
  \multicolumn4c{HARPS-post correction} \\
2457366.76724 & 38.874 & 0.757 & HARPS \\
2457370.79545 & 17.399 & 0.660 & HARPS \\
2457423.63589 & 51.424 & 0.548 & HARPS \\
2457425.63664 & -46.383 & 0.584 & HARPS \\
2457432.68735 & 53.467 & 0.560 & HARPS \\
2457434.59233 & -51.162 & 0.586 & HARPS \\
2457523.58070 & -38.624 & 1.018 & HARPS \\
2457526.57365 & -39.952 & 0.735 & HARPS \\
2457529.55165 & -40.628 & 1.126 & HARPS \\
2457533.49327 & -12.998 & 1.064 & HARPS \\
2457536.53546 & -9.760 & 1.007 & HARPS \\
 \hline
  \multicolumn4c{HIRES/Keck} \\
  2451898.09610 & 22.949 & 1.237 & HIRES \\
2451899.07877 & -53.639 & 1.150 & HIRES \\
2451900.08543 & 37.773 & 1.083 & HIRES \\
2451901.08060 & 18.838 & 1.054 & HIRES \\
2451971.95656 & 48.598 & 1.375 & HIRES \\
2451972.94316 & -3.766 & 1.433 & HIRES \\
2451973.80236 & -54.243 & 1.608 & HIRES \\
2451974.85016 & 48.198 & 1.384 & HIRES \\
2451981.95347 & -6.205 & 1.442 & HIRES \\
2451982.93331 & -48.187 & 1.665 & HIRES \\
2451982.93982 & -40.105 & 1.587 & HIRES \\
2451983.96398 & 52.894 & 1.760 & HIRES \\
2452003.79819 & -39.863 & 1.419 & HIRES \\
2452006.89821 & -34.366 & 1.557 & HIRES \\
2452006.90454 & -29.184 & 1.430 & HIRES \\
2452007.80696 & 56.860 & 1.503 & HIRES \\
2452007.81333 & 55.092 & 1.415 & HIRES \\
2452062.76075 & -32.570 & 1.543 & HIRES \\
2452064.73444 & 58.732 & 1.694 & HIRES \\
2452064.74115 & 59.064 & 1.497 & HIRES \\
2452219.12642 & -10.641 & 1.575 & HIRES \\
2452219.13280 & -11.978 & 1.487 & HIRES \\
2452236.13346 & -46.839 & 1.174 & HIRES \\
2452236.13926 & -46.076 & 1.213 & HIRES \\
2452243.14546 & 0.776 & 1.891 & HIRES \\
2452243.15167 & 0.549 & 1.369 & HIRES \\
2452307.90942 & -51.001 & 1.395 & HIRES \\
2452307.91419 & -54.357 & 1.579 & HIRES \\
2452333.95988 & 22.724 & 1.421 & HIRES \\
2452333.96509 & 23.787 & 1.364 & HIRES \\
2452334.84829 & -56.019 & 1.468 & HIRES \\
2452334.85347 & -52.566 & 1.392 & HIRES \\
2452362.94005 & 41.877 & 1.791 & HIRES \\
2452601.07054 & -32.895 & 1.338 & HIRES \\
2452711.87348 & 10.661 & 1.473 & HIRES \\
2452989.10833 & -43.022 & 1.351 & HIRES \\
2453370.08654 & 13.648 & 1.243 & HIRES \\
2453426.94719 & 5.675 & 1.087 & HIRES \\
2454545.94255 & 57.019 & 1.374 & HIRES \\
2455173.08470 & 12.252 & 1.363 & HIRES \\
2455522.07504 & 30.987 & 1.301 & HIRES \\
2455613.96993 & -11.112 & 1.459 & HIRES \\
2456614.10391 & -3.604 & 1.338 & HIRES \\
2456639.07869 & 26.764 & 1.340 & HIRES \\
2457003.17534 & 23.333 & 3.025 & HIRES \\
   \hline
  \multicolumn4c{AAT} \\
2451212.18299 & -44.95 & 3.90 & AAT \\
2451213.17558 & 16.11 & 3.70 & AAT \\
2451214.27214 & 20.50 & 6.82 & AAT \\
2451682.90876 & 47.91 & 3.56 & AAT \\
2451919.20465 & 17.74 & 4.67 & AAT \\
2451920.18207 & -30.35 & 3.54 & AAT \\
2451983.04402 & -27.82 & 3.99 & AAT \\
2451984.02359 & 60.89 & 4.40 & AAT \\
2452009.08155 & -12.83 & 3.50 & AAT \\
2452060.91795 & 1.98 & 2.85 & AAT \\
2452091.86433 & 77.86 & 4.22 & AAT \\
2452092.88784 & -43.70 & 3.62 & AAT \\
2452127.85212 & 72.24 & 7.42 & AAT \\
2452188.28155 & -25.44 & 1.70 & AAT \\
2452189.27389 & -6.93 & 4.52 & AAT \\
2452359.11623 & -23.39 & 2.62 & AAT \\
2452386.94067 & 71.03 & 2.46 & AAT \\
2452387.94246 & 15.80 & 2.44 & AAT \\
2452389.00130 & -18.86 & 1.69 & AAT \\
2452389.88197 & 66.75 & 2.17 & AAT \\
2452420.95543 & -12.81 & 1.25 & AAT \\
2452421.95680 & -17.54 & 1.57 & AAT \\
2452422.89561 & 66.23 & 1.64 & AAT \\
2456747.08674 & 3.75 & 2.11 & AAT \\
2457095.09367 & 29.60 & 7.76 & AAT \\
%         :        &     :    &   :    & : \vspace{4pt} \\
\enddata
\end{deluxetable}

